Relying on the Metrics of Evaluated Agents

Online platforms and regulators face a continuing problem of designing effective evaluation metrics. While tools for collecting and processing data continue to progress, this has not addressed the problem of "unknown unknowns", or fundamental informational limitations on part of the evaluator. To guide the choice of metrics in the face of this informational problem, we turn to the evaluated agents themselves, who may have more information about how to measure their own outcomes. We model this interaction as an agency game, where we ask: "When does an agent have an incentive to reveal the observability of a metric to their evaluator?" We show that an agent will prefer to reveal metrics that differentiate the most difficult tasks from the rest, and conceal metrics that differentiate the easiest. We further show that the agent can prefer to reveal a metric "garbled" with noise over both fully concealing and fully revealing. This indicates an economic value to privacy that yields Pareto improvement for both the agent and evaluator. We demonstrate these findings on data from online rideshare platforms.

==> sections/abstract/abstract_old.tex <==
With modern availability of data collection and computational tools, firms and policymakers have more flexibility than ever to compute arbitrarily complex metrics to guide decision making. However, a prevailing challenge remains in deciding \textit{which} metrics to compute, where a firm's ability to compute known metrics does not get around the existence of \textit{unknown unknowns}. 
To design better metrics in the face of this information problem, we turn to evaluated agents themselves, who may have more information than a principal about a metric's potential shortcomings or misspecification. We model this interaction as a simple agency game, where we ask, \textit{When does an agent have an incentive to reveal privately observed, cost-correlated information to the principal?}  There are two effects: better information reduces the agent’s information rents but also makes some projects go forward that otherwise would fail. We show that the agent prefers to reveal information that reveals a strong enough differentiation between high and low costs. Expanding the agent’s action space to include the ability to garble their information, we show that under some regularity conditions, the agent always prefers to add some noise to information that would reveal a low cost. Our model has a close analogy to classical price discrimination that allows for exchange of technical insights between the settings.

==> sections/binary_incentives/game_timeline_binary.tex <==
\newcommand{\btspace}{0.0115\textwidth}
\newcommand{\btspacea}{0.105\textwidth}
\newcommand{\btspaceb}{0.21\textwidth + 0.11\textwidth + \btspace}
\newcommand{\btspacec}{0.21\textwidth + \btspace + 0.22\textwidth + 0.075\textwidth + \btspace}
\newcommand{\btspaced}{0.21\textwidth + \btspace + 0.22\textwidth + 0.15\textwidth + 0.065\textwidth + \btspace + \btspace}
\newcommand{\btspacee}{0.21\textwidth + \btspace + 0.22\textwidth + 0.15\textwidth + \btspace + 0.13\textwidth  + 0.07\textwidth}
\newcommand{\btspacef}{0.21\textwidth + 0.22\textwidth + 0.15\textwidth + \btspace + 0.13\textwidth + \btspace + 0.14\textwidth + \btspace + 0.075\textwidth}

\begin{figure*}[!ht]
    \centering
    \begin{tikzpicture}[]
    % draw horizontal line   
    \draw[->] (0,0) -- (\textwidth,0);

    % draw vertical lines
    \foreach \x in {\btspacea,\btspaceb,\btspacec,\btspaced,\btspacee,\btspacef}
      \draw (\x ,3pt) -- (\x ,-3pt);

    % draw nodes
    \draw (\btspacea,0) node[below=3pt] {$t= 0 $} node[above=3pt,text width=0.21\textwidth] 
    {P and A share prior over $C$. \\ \textcolor{gray}{A knows prior joint \\distribution of $C, X$.}} ; % TODO: explain in text that when X is unobservable, reduces to standard agency game.
    \draw (\btspaceb,0) node[below=3pt] {$t= 1 $} node[above=3pt,text width=0.22\textwidth]  
    {\textcolor{gray}{A decides whether to reveal observability of $X$, including joint distribution of $C,X$.}} ;
    \draw (\btspacec,0) node[below=3pt] {$t= 2 $} node[above=3pt,text width=0.15\textwidth] {P offers a contract\textcolor{gray}{, which can depend on $X$ if revealed.}} ; 
    \draw (\btspaced,0) node[below=3pt] {$t= 3 $} node[above=3pt,text width=0.13\textwidth] {\textcolor{gray}{$X$ is realized.}\\ A learns their cost type $C$.} ;
    \draw (\btspacee,0) node[below=3pt] {$t= 4 $} node[above=3pt,text width=0.14\textwidth] {A decides whether or not to accept the contract.} ;
    \draw (\btspacef,0) node[below=3pt] {$t= 5 $} node[above=3pt,text width=0.15\textwidth] {The contract is\\ executed and \\utilities realized.};
    \end{tikzpicture}
    \caption{Timing of the agency game with information transfer between principal (P) and agent (A).}
    \label{fig:timing_revealed}
\end{figure*}

%%% Version with principal joint prior at t=0
% \begin{figure}[!h]
%     \centering
%     \begin{tikzpicture}[]
%     % draw horizontal line   
%     \draw[->] (0,0) -- (13.75,0);

%     % draw vertical lines
%     \foreach \x in {1.35,3.8,6.1,8.4,10.7,12.9}
%       \draw (\x cm,3pt) -- (\x cm,-3pt);

%     % draw nodes
%     \draw (1.35,0) node[below=3pt] {$t= 0 $} node[above=3pt,text width=0.2\textwidth] 
%     {P and A share prior distribution over $C$\textcolor{gray}{, $X$} $\sim \mathcal{D}$.} ; % TODO: explain in text that when X is unobservable, reduces to standard agency game.
%     \draw (3.8,0) node[below=3pt] {$t= 1 $} node[above=3pt,text width=0.15\textwidth]  
%     {\textcolor{gray}{A decides whether or not to reveal observability of $X$.}} ;
%     \draw (6.1,0) node[below=3pt] {$t= 2 $} node[above=3pt,text width=0.15\textwidth] {P offers a \\ contract\textcolor{gray}{, which can depend on $X$ if $X$ observed.}} ; 
%     \draw (8.4,0) node[below=3pt] {$t= 3 $} node[above=3pt,text width=0.15\textwidth] {\textcolor{gray}{$X$ is realized.} A learns their cost type $C$.} ;
%     \draw (10.7,0) node[below=3pt] {$t= 4 $} node[above=3pt,text width=0.15\textwidth] {A decides whether or not to accept the contract.} ;
%     \draw (12.9,0) node[below=3pt] {$t= 5 $} node[above=3pt,text width=0.15\textwidth] {The contract is executed and utilities realized.};
%     \end{tikzpicture}
%     \caption{Timing of the agency game with information transfer between principal (P) and agent (A).}
%     \label{fig:timing_revealed}
% \end{figure}

==> sections/experiments/experiments.tex <==

\section{Experiments}\label{sec:experiments}

% \subsection{Exponential and Weibull Simulation}

% \subsection{Uber and Lyft Pricing Dataset}

To demonstrate how our theory can apply to real scenarios and feature distributions, we turn to public data from the rideshare platforms Uber and Lyft. Platforms like these employ algorithmic pricing methods that depend on numerous ride metrics (or features). We investigate an agent's incentives to reveal features to the platform that would affect their pricing in several hypothetical scenarios. 
%We present hypothetical scenarios constructed using this data
% , with different levels of sophistication for the principal's pricing model.
Our findings track with the intuition built by our theory, and illustrate a variety of agent dynamics that can occur.

% Our analysis using this dataset is not intended as some form of ground truth about rideshare platforms, but instead to demonstrate how our theory applies to feature distributions arising in the wild, as well as a demonstration of scenarios in which our model could be useful to real agents.

\textit{Dataset.} We consider the Uber and Lyft data that is publicly available on Kaggle \cite{uberlyftkaggle}.  This data was scraped using API queries over the course of one week at the end of November, 2018 in Boston, MA. The dataset includes a set of Uber rides and a set of Lyft rides, and contains columns for price, distance, surge multiplier, and others variables. Implementation details are given in Appendix \ref{app:experiments_additional}.

\textit{Scenario: revelation of a highly cost-correlated feature.} Consider a simple scenario in which a competing rideshare company (principal) wants to win over drivers (agents) from Lyft. We use the price column as an approximation for the price offered to the driver. The cost variable $C$ is the price that Lyft offers for the ride, since this is the price that the principal must beat for the driver to switch to the principal's platform. The agent gains utility if the principal offers price $p > C$ to induce the agent to switch; otherwise, the agent ignores the offer and is no worse off than before. Our central question is whether the agent would be better off if the principal offers prices as a function of $X = $ distance, which is highly correlated with $C$. In other words, \textit{would the agent prefer to reveal a highly cost-correlated feature to the initially naive principal?}\footnote{Most real rideshare companies are likely aware of the importance of distance, but for the purposes of this illustration, we consider distance as a stand-in for similarly highly cost-correlated variables.} 
%but this simple illustration should roughly generalize to similarly highly cost-correlated variables. 

\textit{Results.} We analyze the agent's utilities for revealing, concealing, and garbling, and compare with the predictions from our theory. We present results when the principal's value for the agent's switch is $b = 1.5\bar{C}$, such that the prices are not degenerate (e.g., always offering the maximum cost or never offering above some amount).\footnote{A high value of $b$ can be thought of as the principal receiving high reward for winning users to their platform, which is often important to investors. We repeat this for different values of $b$ in the Appendix.} 

First, the agent indeed prefers to reveal the distance feature $X$, with the exact difference in the agent's value between revelation and concealment shown in Figure \ref{fig:lyft_scen1}. This is particularly interesting because a feature which \textit{exactly} matches the cost $C$ would leave the agent with a surplus of $0$. This means that the distance feature is correlated enough with $C$ to change the principal's prices, but adds enough noise to still leave the agent with some surplus. The Pearson correlation between $X$ and $C$ is $\approx 0.36$. 

We now compare this to the agent's incentive to reveal a coarser, binarized version of the distance feature. 
% We consider the agent's incentives to reveal thresholded versions of $X$: 
Let $Z^t = 1$ if $X \leq t$ and $0$ otherwise. This binarized version tracks closely with our theory on thresholding features, as $Z^t$ can be thought of as a noisy thresholding of $C$.
%($Z^t$ thresholds $X$ instead of $C$, and is thus a noisier thresholding of $C$).
Figure \ref{fig:lyft_scen1} shows that for some $t$, the agent actually prefers to reveal $Z^t$ over the full feature $X$. Figure \ref{fig:lyft_scen1} also shows that the agent prefers to conceal $Z^t$ for $t$ very low, and reveal for $t$ is very high, which matches Theorems \ref{thm:reveal_high_t} and \ref{thm:conceal_t}. 

If the agent is further given the chance to \textit{garble} $Z^t$, we show that sometimes the agent prefers garbling over revelation.
%also compute the agent's optimal garbling amount $\veps$ for each binarized feature $Z^t$.
Figure \ref{fig:lyft_scen1} shows the agent's optimal garbling amount $\veps^{*}$ for each $Z^t$. For the highest and lowest thresholds, the agent sticks to either full revelation or full concealment; but for some $t$ in between, the agent achieves even higher utility through garbling than full revelation. As a practical implication, this constitutes a set of scenarios in which an agent derives economic value from feature privacy.

\begin{figure}[!ht]
    \centering
    \begin{tabular}{c}
        Scenario 1: Agent's utility difference for revealing distance\\
        \includegraphics[trim={0.3cm 0.35cm 0 0.25cm},clip, width=\columnwidth]{figures/lyft_scen1_stacked.pdf}
    \end{tabular}
    \caption{Agent's utility differences for revealing the distance feature (positive means the agent prefers to reveal). The dotted line is the agent's value difference upon revealing the full distance feature $X$. The \textcolor{blue}{solid blue line} shows the agents value differences upon revealing $Z^t$ for different thresholds $t$. The \textcolor{orange}{dashed orange line } shows the agent's value difference upon revealing the optimal garbled version of $Z^t$, for optimal garbling parameter $\veps^{*}$ displayed above ($\veps = 1$ corresponds to full revelation, and $\veps = 0$ to full concealment). In alignment with our theory, the agent prefers to conceal for $t$ low enough, and reveal for $t$ high enough. There also exist $t$ values in the middle in which \textcolor{orange}{garbled} > \textcolor{DarkGreen}{revealed} > \textcolor{red}{concealed}.}
    \label{fig:lyft_scen1}
\end{figure}



\textit{Discussion and Limitations.} The findings from this scenario give a rough picture of the types of features that an agent would want to reveal given this data. In Appendix \ref{app:scen2}, we construct a second similar scenario in which the principal starts with a more sophisticated baseline pricing model, which yields similar results. In general, these are not intended as a characterization of real rideshare platforms, but instead as a demonstration of how our model can be applied to analyze metric elicitation incentives in practical settings. For example, a collective action organization acting on behalf of drivers might perform analysis like the above, and determine whether it would be beneficial to reveal new, possibly garbled or thresholded features to a rideshare platform. We encourage replication of similar analyses by agencies with internal data sources.
% On the other hand, in practice, agents may have to work with coarser versions of data and estimates of pricing models when making real decisions, and further exploration of the consequences of the agent having imperfect information would also be interesting to explore.

% Even with the extra features in the pricing model in Scenario 2, this is still far from capturing the full complexity of real dynamic pricing models. In general, the findings from Scenarios 1 and 2 are not intended to be taken as some form of ground truth about rideshare platforms, but instead as a demonstration of how our model can be applied to analyze metric elicitation incentives in practical settings. For example, a collective action organization acting on behalf of drivers might perform analysis like in Scenario 2, and determine whether it would be beneficial to reveal new, possibly garbled or thresholded features to the principal. To make any real decisions, we highly encourage replication of similar analyses by agencies with internal data sources.


% but instead as a demonstration of this is not intended to be interpreted In general, our intention for our analysis in Scenarios 1 and 2 is to be viewed as a demonstration of how our model can be applied to analyze metric elicitation incentives in practical settings for online platforms, rather than to be taken as a ground truth. We encourage replication of similar analyses by agencies with internal data sources.




==> sections/garbling/game_timeline_garbling.tex <==
\newcommand{\tspace}{0.0115\textwidth}
\newcommand{\tspacea}{0.105\textwidth}
\newcommand{\tspaceb}{0.21\textwidth + 0.11\textwidth + \tspace}
\newcommand{\tspacec}{0.21\textwidth + \tspace + 0.22\textwidth + 0.06\textwidth + \tspace}
\newcommand{\tspaced}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.065\textwidth + \tspace}
\newcommand{\tspacee}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.13\textwidth + \tspace + 0.07\textwidth + \tspace}
\newcommand{\tspacef}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.13\textwidth + \tspace + 0.14\textwidth + \tspace + 0.075\textwidth + \tspace}


\begin{figure*}[!ht]
    \centering
    \begin{tikzpicture}[]
    % draw horizontal line   
    \draw[->] (0,0) -- (\textwidth,0);

    % draw vertical lines
    \foreach \x in {\tspacea,\tspaceb,\tspacec,\tspaced,\tspacee,\tspacef}
      \draw (\x ,3pt) -- (\x ,-3pt);

    % draw nodes
    \draw (\tspacea,0) node[below=3pt] {$t= 0 $} node[above=3pt,text width=0.21\textwidth] 
    {P and A share prior over $C$. \textcolor{gray}{A knows prior joint \\distribution of $C, X$.}} ;  
    \draw (\tspaceb,0) node[below=3pt] {$t= 1 $} node[above=3pt,text width=0.22\textwidth]  
    {\textcolor{gray}{A selects $\veps$, and reveals \\ observability of $Y$, including joint distribution of $C,Y$.}} ;
    \draw (\tspacec,0) node[below=3pt] {$t= 2 $} node[above=3pt,text width=0.12\textwidth] {P offers a \\
    contract\textcolor{gray}{, which depends on $Y$.}} ;
    \draw (\tspaced,0) node[below=3pt] {$t= 3 $} node[above=3pt,text width=0.13\textwidth] {\textcolor{gray}{$X$ and $Y$ are \\ realized.} A learns their cost type $C$.} ;
    \draw (\tspacee,0) node[below=3pt] {$t= 4 $} node[above=3pt,text width=0.14\textwidth] {A decides whether or not to accept the contract.} ;
    \draw (\tspacef,0) node[below=3pt] {$t= 5 $} node[above=3pt,text width=0.15\textwidth] {The contract is \\executed and\\ utilities realized.};
    \end{tikzpicture}
    \caption{Timing of the agency game with \textit{garbled} information transfer between principal (P) and agent (A).}
    \label{fig:timing_garbled}
\end{figure*}

==> sections/garbling/garbling.tex <==
\section{Information Revelation with Garbling}\label{sec:garbling}

So far, we have compared the settings when $X$ is either concealed or  revealed, focusing on the agent's incentive to induce each setting at time $t=1$. We now generalize the agent's action space to instead be able to reveal a \textit{garbled} version of the variable $X$. 
The agent's garbling action space interpolates between the concealed and revealed settings. We consider a \textit{randomized response} garbling mechanism, which is a noise addition method that has been applied in many settings, from statistical informativeness \citep{blackwell1951comparison} to survey experiment design \citep{warner1965randomized} to differential privacy \citep{dwork2006calibrating,kasiviswanathan2011can}. In particular, we formally show that our garbling mechanism guarantees a notion of differential privacy with respect to an agent's metric value $X$.

As an overview of results in this section, we show that there exist conditions under which the agent would prefer to garble over both concealment and revelation. Thus, having the option to garble can benefit the agent, and even induce the agent to reveal more information when they would otherwise fully opt to conceal $X$, thus leading to a Pareto improvement for both the principal and agent. We also show that garbling improves total welfare over the concealed setting.

\subsection{Agency Game with Garbling} Suppose the agent has the option to present the principal with a different variable $Y$ with noise added to the binary variable $X$:
%\\ $Y = \{
    % X \; \text{w.p. } \varepsilon; \;\;
    % \xi  \; \text{w.p. } 1 - \varepsilon \}$,
\begin{equation*}\label{eq:Y}
    Y = \begin{cases}
    X & \text{w.p. } \varepsilon \\
    \xi &\text{w.p. } 1 - \varepsilon,
\end{cases} 
\end{equation*}
where $\xi \sim \text{Bernoulli}(\theta)$  is independent of $X$ and $C$, for $\theta = \sP(X = 1)$. For ease of exposition, we focus on binary $X$ and $Y$, though further extensions with different noise models can be made for continuous $X$. 
%, and we expect that the general insights will transfer. % The marginal distribution of $Y$ is the same as that of $X$ if and only if $\gamma = \theta$.  

The game with garbling proceeds as before, but the agent selects $\veps \in [0,1]$ at time $t=1$. The full timing is outlined in Figure \ref{fig:timing_garbled}. The agency game with garbled information transfer is a generalization of the previous game: in the previous timing in Figure \ref{fig:timing_revealed}, the agent's choice at $t=1$ would be equivalent to selecting $\veps$ from a more restricted set $\{0,1\}$. In other words, garbling \textit{interpolates} between the concealed and revealed settings in the previous game.

% \begin{figure}[!h]
%     \centering
%     \begin{tikzpicture}[]
%     % draw horizontal line   
%     \draw[->] (0,0) -- (13.75,0);

%     % draw vertical lines
%     \foreach \x in {1.35,3.8,6.2,8.4,10.7,12.9}
%       \draw (\x cm,3pt) -- (\x cm,-3pt);

%     % draw nodes
%     \draw (1.35,0) node[below=3pt] {$t= 0 $} node[above=3pt,text width=0.2\textwidth] 
%     {P and A share prior distribution over $C$\textcolor{gray}{, $X, \xi$} $\sim \mathcal{D}$.} ;  
%     \draw (3.8,0) node[below=3pt] {$t= 1 $} node[above=3pt,text width=0.15\textwidth]  
%     {\textcolor{gray}{A selects $\veps$, and reveals observability of $Y$ (\ref{eq:Y})}} ;
%     \draw (6.2,0) node[below=3pt] {$t= 2 $} node[above=3pt,text width=0.15\textwidth] {P offers a \\ contract\textcolor{gray}{, which depends on $Y$.}} ;
%     \draw (8.4,0) node[below=3pt] {$t= 3 $} node[above=3pt,text width=0.15\textwidth] {\textcolor{gray}{$X$ and $Y$ are realized.} A learns their cost type $C$.} ;
%     \draw (10.7,0) node[below=3pt] {$t= 4 $} node[above=3pt,text width=0.15\textwidth] {A decides whether or not to accept the contract.} ;
%     \draw (12.9,0) node[below=3pt] {$t= 5 $} node[above=3pt,text width=0.15\textwidth] {The contract is executed and utilities realized.};
%     \end{tikzpicture}
%     \caption{Timing of the agency game with \textit{garbled} information transfer between principal (P) and agent (A).}
%     \label{fig:timing_garbled}
% \end{figure}

\newcommand{\tspace}{0.0115\textwidth}
\newcommand{\tspacea}{0.105\textwidth}
\newcommand{\tspaceb}{0.21\textwidth + 0.11\textwidth + \tspace}
\newcommand{\tspacec}{0.21\textwidth + \tspace + 0.22\textwidth + 0.06\textwidth + \tspace}
\newcommand{\tspaced}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.065\textwidth + \tspace}
\newcommand{\tspacee}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.13\textwidth + \tspace + 0.07\textwidth + \tspace}
\newcommand{\tspacef}{0.21\textwidth + \tspace + 0.22\textwidth + 0.12\textwidth + \tspace + 0.13\textwidth + \tspace + 0.14\textwidth + \tspace + 0.075\textwidth + \tspace}


\begin{figure*}[!ht]
    \centering
    \begin{tikzpicture}[]
    % draw horizontal line   
    \draw[->] (0,0) -- (\textwidth,0);

    % draw vertical lines
    \foreach \x in {\tspacea,\tspaceb,\tspacec,\tspaced,\tspacee,\tspacef}
      \draw (\x ,3pt) -- (\x ,-3pt);

    % draw nodes
    \draw (\tspacea,0) node[below=3pt] {$t= 0 $} node[above=3pt,text width=0.21\textwidth] 
    {P and A share prior over $C$. \textcolor{gray}{A knows prior joint \\distribution of $C, X$.}} ;  
    \draw (\tspaceb,0) node[below=3pt] {$t= 1 $} node[above=3pt,text width=0.22\textwidth]  
    {\textcolor{gray}{A selects $\veps$, and reveals \\ observability of $Y$, including joint distribution of $C,Y$.}} ;
    \draw (\tspacec,0) node[below=3pt] {$t= 2 $} node[above=3pt,text width=0.12\textwidth] {P offers a \\
    contract\textcolor{gray}{, which depends on $Y$.}} ;
    \draw (\tspaced,0) node[below=3pt] {$t= 3 $} node[above=3pt,text width=0.13\textwidth] {\textcolor{gray}{$X$ and $Y$ are \\ realized.} A learns their cost type $C$.} ;
    \draw (\tspacee,0) node[below=3pt] {$t= 4 $} node[above=3pt,text width=0.14\textwidth] {A decides whether or not to accept the contract.} ;
    \draw (\tspacef,0) node[below=3pt] {$t= 5 $} node[above=3pt,text width=0.15\textwidth] {The contract is \\executed and\\ utilities realized.};
    \end{tikzpicture}
    \caption{Timing of the agency game with \textit{garbled} information transfer between principal (P) and agent (A).}
    \label{fig:timing_garbled}
\end{figure*}

The principal treats the variable $Y$ as a revealed metric with prior joint distribution $Y, C$, and proceeds to design the optimal contract conditioning on $Y$. This is optimal for the principal both in the case where the principal has no knowledge of $\veps$ or $X$, and in the case where the principal knows $\veps$ and the joint distribution of $C,X$ (but not the realized value of $X$).
% \footnote{The simplest way to think of this is that the principal does not learn of the existence of $X$ after $Y$ is revealed. In practice, this would also be equivalent to the principal agreeing to maintain a noise level $\veps$ requested by the agent as a policy.}
%It is assumed that the principal either cannot or agrees not to attempt to back out $\veps$ or the previous value of $X$.

The game proceeds as delineated for the revealed information contract in Section \ref{sec:revealed}, but using the variable $Y \in \mathcal{Y}$ instead of $X$. Specifically, the principal designs a contract with prices $\rho: \mathcal{Y} \to \mathbb{R}_{+}$,
and upon execution of the contract, the agent receives payment $\rho(y)$ if they exert effort and $Y=y$. 

The principal's utility under revelation of a given garbled variable $Y$ is $\Vpeps(\rho) \coloneq E[(b - \rho(Y))\Ind(C < \rho(Y))]$,
and the agent's utility is
$\Vaeps(\rho) \coloneq E[(\rho(Y)-C)\Ind(C < \rho(Y))]$. After $Y$ is revealed, the principal selects $\rho^{*} \in \arg\max_{\rho \in \mathcal{F}} \Vpeps(\rho)$. 
% Binary version:
% \begin{align*}%\label{eq:principal_V_eps}
%     \Vpeps(p_0, p_1) = (1-\theta)&E[(b - p_0)\Ind(C < p_0)| Y = 0] \\
%     +\; \theta &E[(b - p_1)\Ind(C < p_1)| Y = 1],
% \end{align*}
% and the utility of the agent is given by
% \begin{align*}%\label{eq:agent_V_eps}
%     \Vaeps(p_0, p_1) = (1-\theta) &E[(p_0 - C)\Ind(C < p_0) | Y = 0] \\+\; \theta &E[(p_1 - C) \Ind(C < p_1) | Y = 1].
% \end{align*}

For a given $\veps$ chosen at $t=1$, we denote the equilibrium utilities as $\Vpeps(\veps) = \Vpeps(\rho^{*}), \Vaeps(\veps) = \Vaeps(\rho^{*})$. The agent's optimal choice of $\veps$ at time $t=1$ is then $\veps^{*} \in \arg\max_{\veps \in [0,1]} \Vaeps(\veps)$. An optimal choice of $\veps^{*} = 0$ corresponds to full concealment, and $\veps^{*} = 1$ corresponds to full revelation. In the following sections, we analyze the effects of this optimal choice on welfare, and compare this to the welfare effects of the agent's optimal choice in the previous game without the garbling option. We also formally connect the garbling model to existing notions of differential privacy.

% The garbling model also provides privacy guarantees for the agent's metric $X$, which we formalize below as well.
%\[\Vpeps(\veps) = \Vpeps(p_0(\veps), p_1(\veps)), \;\; \Vaeps(\veps) = \Vaeps(p_0(\veps), p_1(\veps)). \]

\subsection{Agent's Garbling Incentives}\label{sec:agent_garbling}


Our primary observation is that even for distributions satisfying the regularity conditions from before, there exist cases when some amount of garbling is preferred over both concealment and revelation, for \textit{both} orderings of concealment vs. revelation. That is, there exist settings when $\textcolor{orange}{\Vaeps(\veps^{*})} > \textcolor{DarkGreen}{\Var(\rho^{*})} > \textcolor{red}{\Vah(p^{*})} $ (a.k.a. \textcolor{orange}{garbled} > \textcolor{DarkGreen}{revealed} > \textcolor{red}{concealed}), and settings when $\textcolor{orange}{\Vaeps(\veps^{*})}  > \textcolor{red}{\Vah(p^{*})} > \textcolor{DarkGreen}{\Var(\rho^{*})}$ (\textcolor{orange}{garbled} > \textcolor{red}{concealed} > \textcolor{DarkGreen}{revealed}).

Both orderings are significant from a policy standpoint. The case when \textcolor{orange}{garbled} > \textcolor{DarkGreen}{revealed} > \textcolor{red}{concealed} is interesting since it indicates that the agent derives economic value from adding noise to their data compared to fully revealing. 
% notion of privacy compared to fully revealing their data. 
Thus, \textit{even without any inherent value for privacy, the agent still prefers the privatized setting}.

The case when \textcolor{orange}{garbled} > \textcolor{red}{concealed} > \textcolor{DarkGreen}{revealed} is perhaps even more interesting, since without the ability to only partially reveal a garbled $Y$, the agent would have otherwise chosen to conceal. Thus, allowing for garbling results in a strict Pareto improvement for both the principal and agent; that is, \textit{both principal and agent benefit from the option of privacy}. This provides an incentive for a platform to agree to maintain garbling of a feature, even if they could otherwise discover $X$ after $Y$ is revealed. 

Figure \ref{fig:expon_garbling_stacked} illustrates a continuum of distributions that contain both of these orderings. Specifically, let $C$ be a mixture of exponentials with $C | X = 0 \sim \text{Exp}(\frac{1}{\lambda_0})$ and $C | X = 1 \sim \text{Exp}(\frac{1}{\lambda_1})$, where $\lambda_x$ is the mean of the distribution. Fixing $\theta = \frac{1}{2}$, $b = 1$, and $\lambda_0 = 0.5$, Figure \ref{fig:expon_garbling_stacked} shows a range of $\lambda_1$ in which the agent prefers \textcolor{orange}{garbled} > \textcolor{red}{concealed} > \textcolor{DarkGreen}{revealed}, and as $\lambda_1$ increases, this flips to \textcolor{orange}{garbled} > \textcolor{DarkGreen}{revealed} > \textcolor{red}{concealed}. Thus, even within the same family of ``nice'' distributions, both orderings can occur.

\begin{figure}[!ht]
    \centering
    \begin{tabular}{c}
        Agent's value difference for a mixture of exponentials \\
        \includegraphics[trim={0.3cm 0.35cm 0 0.25cm},clip, width=\columnwidth]{figures/expon_garbling_sim_stacked.pdf}
    \end{tabular}
    \caption{Agent's utility differences for revealing $X$ and garbled $Y$ when $C$ is a mixture of exponentials. We fix $\theta=\frac{1}{2}$, $b = 1$, and $\lambda_0 = 0.5$, and vary $\lambda_1$. 
    The \textcolor{blue}{solid blue line} shows the agents utility difference upon revealing $X$ for each value of $\lambda_1$. The \textcolor{orange}{dashed orange line } shows the agent's utility difference upon revealing the optimal garbled $Y$, for optimal garbling parameter $\veps^{*}$ displayed above. This first lighter shaded region highlights settings where \textcolor{orange}{garbled} > \textcolor{red}{concealed} > \textcolor{DarkGreen}{revealed}. The second darker shaded region highlights settings where \textcolor{orange}{garbled} > \textcolor{DarkGreen}{revealed} > \textcolor{red}{concealed} .
    }
    \label{fig:expon_garbling_stacked}
\end{figure}

% For the agent, there is no clear ordering between $\Vaeps(p_0(\veps), p_1(\veps))$, $\Vah(p^{*})$, and $\Var(p_0^{*}, p_1^{*})$. 
% Garbling can be better for the agent than concealment, even when hiding is preferred  over revelation, $\Vah(p^{*}) > \Var(p_0^{*}, p_1^{*})$. Garbling can also be better than revelation, even when revelation is preferred over hiding,  $\Vah(p^{*}) < \Var(p_0^{*}, p_1^{*})$. We illustrate both of these cases using exponential distributions in Section \ref{sec:weibull_garbling}, as previously done for the full concealment and revelation comparison in Section \ref{sec:weibull}.

To give a more general theoretical characterization of the agent's garbling incentives, we give sufficient conditions for the agent to prefer a nonzero amount of garbling over full revelation in Appendix \ref{app:garbling_general}. This can be seen as a softer version of the previous analysis of when the agent prefers full concealment over full revelation.


\subsection{Garbling and Total Welfare}\label{sec:garbling_total_welfare}

We next show that garbling increases total welfare ($\Vjeps(\veps) \coloneqq \Vpeps(\veps) + \Vaeps(\veps)$) relative to concealment. The principal always benefits from more information, which we formalize in \ref{sec:principal_garbling}. Optimal garbling always increases total welfare over concealment. A more subtle finding is that adding a marginal amount of garbling compared to concealment \textit{also} increases total welfare. 

% We now discuss the relationship between the agent's the choice of garbling amount $\veps$ and total welfare, $\Vjeps(\veps) \coloneqq \Vpeps(\veps) + \Vaeps(\veps).$ 

First, we show that the \textit{optimal} amount of garbling chosen by the agent also increases total welfare over the fully concealed setting.

\begin{lemma}[Optimal garbling increases welfare over concealment]\label{lem:total_welfare_opt_garbling}
    Let $\veps^{*} \in \arg\max_{\veps \in [0,1]} \Vaeps(\veps)$. Then $\Vjeps(\veps^{*}) \geq \Vjeps(0)$. 
\end{lemma}

Intuitively, Lemma \ref{lem:total_welfare_opt_garbling} follows from the fact that the principal is never hurt by additional information (formalized in Appendix \ref{sec:principal_garbling}). Given that the agent benefits from their optimal garbling choice, total welfare must increase. 

Next, we show that relative to the fully concealed setting, the marginal effect of revealing any information on total welfare is initially positive relative to full concealment. 
%Relative to full concealment with $\veps = 0$, revealing $Y$ with some garbled noise initially does not decrease total welfare.

% \begin{align*}
%     4 \frac{\partial}{\partial \veps} \Vjeps= &\underset{\text{\textcolor{red}{Positive}}}{\left(\Pi_0'(p_0^{\veps}) - \Pi_1'(p_0^{\veps})\right)} z_0^{\veps}(p_0^{\veps}) + \underset{\text{\textcolor{red}{Negative}}}{\left(\Pi_1'(p_1^{\veps}) - \Pi_0'(p_1^{\veps})\right)}z_1^{\veps}(p_1^{\veps}) \\
%     &+ \underset{\text{\textcolor{red}{Welfare dominance, usually negative?}}}{\left((W_0(p_0^{\veps}) - W_0(p_1^{\veps})) - (W_1(p_0^{\veps}) - W_1(p_1^{\veps}))\right)} \\
% \end{align*} 

\begin{lemma}[More information initially increases welfare]\label{lem:total_welfare_zero_deriv}
    Increasing $\veps$ from $0$ marginally increases total welfare: $\Vjeps'(0) \geq 0$. The inequality is strict if $\Vpeps'(0) > 0$.
    %, which is true under strict concavity of $\Pi_0(p), \Pi_1(p)$ (Assumption \ref{assn:concave}) and MLRP (Assumption \ref{assn:mlrp}).
\end{lemma}

While the agent's chosen amount of garbling $
\veps^{*}$ improves total welfare over concealment, the question remains of where $
\veps^{*}$ falls relative to the optimal amount of garbling that maximizes total welfare. 
Lemma \ref{lem:garbling_total_welfare_derivative} shows that the optimal amount of garbling that maximizes total welfare must necessarily reveal at least as much information as the optimal amount of garbling chosen by the agent. 
%Under Assumptions \ref{assn:concave} and \ref{assn:mlrp}, if $\veps^{*} < 1$, then the $\veps$ that maximizes total welfare is strictly higher than the $\veps$ that maximizes agent utility.

\begin{lemma}[More information increases total welfare relative to agent optimal garbling]\label{lem:garbling_total_welfare_derivative} $\Vjeps'(\veps) \geq \Vaeps'(\veps)$ for all $\veps \in [0,1]$. The inequality is strict if $\Vpeps'(0) > 0$.
%which is true under strict concavity of $\Pi_0(p), \Pi_1(p)$ (Assumption \ref{assn:concave}) and the MLRP (Assumption \ref{assn:mlrp}).
\end{lemma}

The benefits of garbling to total welfare have interesting policy implications, as the increase in total welfare means that a third party designer could inject garbling noise (perhaps for privacy reasons), and later redistribute surplus such that both principal and agent do not end up with worse utilities. We next formalize the connection between garbling and notions of differential privacy.

\input{sections/garbling/garbling_and_dp}


==> sections/model/model.tex <==
\section{Agency Game with Information Transfer}

To gain insight into the incentives surrounding the discovery of metrics, we start with a standard agency game in which a principal contracts an agent to complete a task. In such a game, we ask, \textit{when does the agent have an incentive to reveal observability of a cost-correlated variable to the principal?} 

Specifically, suppose a principal contracts the agent to complete a task, where an agent may exert binary effort. Suppose the principal receives value $b$ if the agent exerts effort and completes the task, and $0$ otherwise (we assume that the task is completed deterministically if the agent exerts effort). Suppose the agent incurs cost $C \in \mathbb{R}_{+}$ for exerting effort. The exact cost is unobserved to the principal, but the principal is aware of a prior distribution over agent's cost type, denoted by the random variable $C$. The agent observes both the proposed price and their realized cost type before deciding whether or not to exert effort. This maps onto the well-established agency game setup where the principal must design a contract when the agent's cost and effort are private \citep{laffont1986using}.
%overall market value of the task, including what an agent would be offered on an open market for LLM queries, or what an agent would be paid if they were to complete the task for a different principal, or the price they would be offered on the open market with outside options beyond the specific contract offered by the principal.
%For simplicity, we focus on uncertain cost and ignore the uncertainty between effort and task completion.

To model the agent's additional knowledge of a metric, suppose the agent is aware of a variable $X \in \mathcal{X}$ which is correlated with their cost $C$. 
% The question of knowledge of $X$ becomes significant when $X$ is correlated with $C$. 
However, $X$ is an \textit{unknown unknown} to the principal. Prior to the principal's design of the contract, the agent has a choice of whether or not to \textit{reveal} $X$, which entails revealing both the \textit{observability} of $X$ at the time of the design of the contract, and the realized \textit{value} of $X$ at the execution of the contract (which the principal can verify). 
The fact that $X$ is not observable to the principal without the agent revealing is a key distinction between our model and prior work in signaling games. That is, the principal cannot rely on prior information over $C$ and $X$, since they are not even aware of the \textit{existence} of $X$. This allows us to analyze a decision problem that differs from that of the standard Bayesian framework, which instead focuses on an agent's decision to reveal their \textit{value} of $X$ after it is realized.


% \textcolor{blue}{A second distinction between our model and existing persuasion games is that the agent cannot selectively reveal the value of $X$ once observability has been established. All of the agent's decisions must be made prior to the realization of their actual values, and we assume a principal powerful enough to observe the actual value of $X$ once revealed. This reflects a common reality in online platforms, where the platform often has significant data collection power. It also reflects a setting where the platform or government can even compel an evaluated agent to report metrics \cite{dranove2003more}. 
% \footnote{It would be possible to extend our model to include an extra decision step for the agent after observability of $X$ is revealed, which would be an interesting combination of our question with existing work in persuasion games, and an interesting grey area to explore in the balance of power between platforms and users.}


If the agent chooses to not reveal $X$, then the rest of the game proceeds as a standard agency game with private cost: the principal designs a contract based on their knowledge of the prior distribution $C$.
If the agent reveals $X$, then the principal can offer a contract that conditions on the realized value of $X$. 
%We assume that the agent cannot change the joint distribution of $C,X$. 
The timing of the full agency game with the possibility of agent information transfer is summarized in Figure \ref{fig:timing_revealed}. The text in black matches the standard agency game \citep{laffont1986using}, and the text in \textcolor{gray}{gray} represents additional elements introduced by our model.

\input{sections/binary_incentives/game_timeline_binary}

%In our simplified agency game with binary effort,
The principal's contract design problem when $X$ is concealed reduces to choosing a single price $p$ where the agent is paid $p$ if the task is completed, and zero otherwise. If $X$ is revealed, then the principal offers a contract with distinct prices $\rho(x)$ for different realized values of $x \in \mathcal{X}$. At the execution of the contract, the agent receives payment $\rho(x)$ if the task is completed and $X = x$, and $0$ otherwise. 
We assume that the principal still receives the same value $b$ if the task is completed, regardless of $X$. 

The key question in this work concerns the agent's decision of whether or not to 
% inform the principal of the existence of 
reveal $X$ at time $t=1$. In Section \ref{sec:binary}, we treat this as a binary decision of whether or not to reveal $X$; we will later relax this in Section \ref{sec:garbling} to expand the agent's action space to reveal a garbled version of $X$, thus interpolating between the concealed and revealed settings.

\subsection{Optimal Contracts}\label{sec:utilities}

We begin by outlining the optimal contract and equilibrium utilities of the principal and agent when the contract is agnostic of $X$, which we refer to as the \textit{concealed information} setting. Then, we outline the optimal contract and equilibrium utilities when the principal can condition on $X$ to determine payments to the agent, which we refer to as the \textit{revealed information} setting. We assume that both principal and agent are risk neutral throughout.

% We set up this problem by first outlining the contract and equilibrium behavior of the principal and agent without information transfer, which we refer to as the \textit{hidden information} setting. Then, we outline the contract when the principal can condition on $X$ to determine payments to the agent, which we refer to as the \textit{revealed information} setting. Later sections will analyze when each setting is better for the principal and/or agent.

\textit{Concealed information contract.}
If the metric $X$ is not revealed at $t=1$, then the rest of the game proceeds as a standard agency game with private cost, where the principal chooses a single transfer $p$ based on their knowledge of the prior distribution over the agent's cost $C$.
The agent's optimal policy at the execution of the contract is to exert effort if their realized cost is less than or equal to the payment. Thus, the agent's best response to the principal's choice of transfer $p$ is to exert effort with probability $F(p) = \sP(C \leq p)$ (the set where $C = p$ has measure zero).\footnote{We may also think of $F(p)$ as the task completion ``quantity'' as a function of price $p$, or the proportion of agents drawn uniformly at random from a population with costs distributed as $C$ that would complete the task for price $p$.}

For a given choice of transfer $p$, the principal's expected utility when $X$ is hidden is given by $\Vph(p) \coloneqq F(p)(b - p)$.
The agent's expected utility under the principal's choice of transfer $p$ is given by
$\Vah(p) \coloneqq \E[(p - C) \Ind(C < p)]$.
%\label{eq:vah}
%= \int_{0}^{p^{*}} (p^{*} - c) f(c) dc.
The principal moves first and chooses $p^{*} \in \arg\max_{p \geq 0} \Vph(p)$. The agent's utility at equilibrium is then $\Vah(p^{*})$.
% First order conditions give that $p^{*}$ satisfies
% \begin{equation}\label{eq:opt_p_x-hidden}
%     f(p^{*}) (v - p^{*}) = F(p^{*}) \implies p^{*} + \frac{F(p^{*})}{f(p^{*})} = v.
% \end{equation}

% We may think of $C$ as the agent's type, or production efficiency. We assume that the agent does not get to know their type before accepting the contract. However, they do realize their type $C$ before choosing whether or not to perform the task.

\textit{Revealed information contract.}\label{sec:revealed} If the metric $X$ is revealed at time $t=1$, then the principal can vary the payment amount depending on $X$, denoted as $\rho: \mathcal{X} \to \R_{+}$. 
%Since the agent is aware of the values of both $C$ and $X$ before deciding whether to exert effort, and there is no possibility to lie about $X$,
% The agent's optimal policy is to exert effort if their realized cost is no greater than the transfer given the realized $X$ value. Therefore,
The agent's best response to the principal's payment function $\rho(\cdot)$ is to exert effort with probability $F_x(\rho(x))$ when $X = x$.
The principal's expected utility in the revealed setting is given by
$\Vpr(\rho) \coloneqq \E[F_X(\rho(X))(b - \rho(X))]$, maximized at $\rho^{*} \in \arg\max_{\rho \in \mathcal{F}} \Vpr(\rho)$.
% More detailed version:
% \begin{equation*}
%     \Vpr(\rho) \coloneqq \E[F_X(\rho(X))(b - \rho(X))] = \E[\Pi_X(\rho(X))], 
% \end{equation*}
% where $\Pi_x(p) \coloneqq F_x(p)(b-p)$. 
The agent's expected utility under the principal's choice of transfer function $\rho(\cdot)$ is then $\Var(\rho) \coloneqq \E[(\rho(X) - C)\Ind(C < \rho(X))]$.
% More detailed version:
% \begin{equation*}\label{eq:agent_revealed}
%     \Var(\rho) \coloneqq \E[(\rho(X) - C)\Ind(C < \rho(X))] = \E[V_X(\rho(X))],
% \end{equation*}
% where $V_x(p) \coloneqq \E[(p-c)\Ind(C < p) | X = x]$.
The agent's choice of whether to reveal or conceal is ultimately determined by their \textit{utility difference}, $\Var(\rho^{*}) - \Vah(p^{*})$.

% In the following sections, we will analyze the effects of information revelation on the agent's utility, principal's utility, and total welfare. 
%We will empirically evaluate some of these effects and utilities on real data in Section \ref{sec:experiments}.
%Specifically, we will compare $\Vah(p^{*})$ to $\Var(p_0^{*}, p_1^{*})$ to understand the agent's incentive to reveal $X$. We will also analyze the consequences of the agent's revelation decision on the principal's utility, as well as consequences on total welfare. 

==> sections/price_discrimination.tex <==
\section{Mapping to price discrimination}

Our model has a close analog to price discrimination in multiple independent markets. Here we show this mapping in detail, and suggest a translation and interpretation of our garbling insights in the price discrimination setting.

Mirroring the setup from \citet{mcafeepricing}, suppose we have $n$ markets, and the firm sets prices $\mathbf{p} = \{p_1,...,p_n\}$. We suppose all markets are independent and unaffected by the prices in other markets, so each market demands $q_i(p) \in [0,1]$. The demand $q_i(p)$ represents a distribution over consumer types, where $q_i(p)$ is the proportion of consumers who would purchase the good for price at least $p$. The total size of each market $i$ is given by $\theta_i \in [0,1]$, with $\sum_{i=1}^n \theta_i = 1$. The total profit of the firm is given by
\[V = \sum_{i=1} (p_i - mc)\theta_i q_i(p_i), \]
where the marginal cost $mc$ is assumed constant. The non-discriminating monopolist would charge the same price in all markets $p_i = p^{*} \;\forall i \in \{1,...,n\}$. The discriminating monopolist charges different prices $p_i^{*}$ in each market.

The analogous quantities to our setting are: 
\begin{itemize}
    \item The constant marginal cost $mc$ is analogous to the negative of the constant marginal value $v$ that the principal gains per completed task. 
    \item $p_i$ is analogous to the negative of the payment that the principal offers agent $i$ for completing the task.
    \item The demand distribution $q_i(p)$ is analogous to the cost distribution $F_i(p)$, which is the proportion of agents who would complete the task if paid at least $p$. $q_i(p)$ is decreasing in $p$, whereas $F_i(p)$ is increasing in $p$.
\end{itemize}

The non-discriminating monopolist is analogous to a principal without information $X$. The discriminating monopolist is analogous to a principal that sets different payments depending on $X$.

Garbling in the price discrimination setting would be akin to blending the markets. Instead of distinct market demands $q_1(p), q_2(p)$, a firm under garbling would observe market demands $\tilde{q}_1(p), \tilde{q}_2(p)$, where 
    \[\tilde{q}_1(p) = \frac{1 + \veps}{2} q_1(p) + \frac{1 - \veps}{2} q_2(p); \quad \tilde{q}_2(p) = \frac{1 + \veps}{2} q_2(p) + \frac{1 - \veps}{2} q_1(p). \]
    For $\veps = 0$, there would be no distinction between the markets anymore: $\tilde{q}_1(p) = \tilde{q}_2(p)$.     
Analysis from or similar to Section \ref{sec:garbling} would thus determine when the consumer would prefer for the firm to have garbled market demands.
% The analogous result would be that if a consumer doesn't know which market they will end up in ex ante, and some markets would maintain high demand at very high prices, then the consumer would prefer for the firm to have garbled market demands.

==> sections/trajectories.tex <==
\section{Surplus Trajectories and the Limits of Price Discrimination}

Related work by \citep{bergemann2015limits} characterizes the limits of consumer, producer, and joint surpluses for all possible market segmentations under price discrimination. A market segmentation corresponds with the principal's segmentation of payments $p_x$ for different realized values of an agent's feature $X$. Our work differs in that we consider outcomes when the agent has control over the revelation policy. Instead of looking at all possible segmentations, we consider the agent's information revelation incentives as a function of the properties of a specific segmentation induced by a feature $X$ which is initially only available to the agent. We further plot the trajectories of principal value and agent value as a function of the amount of noise that the agent adds. 

\subsection{Limits of price discrimination}

We begin by plotting the surplus triangle in Figure \ref{fig:surplus-triangle} from \citep{bergemann2015limits}. The shaded area represents the maximal feasible set of principal and agent value combinations, where a combination ($\Pi$, $V$) is feasible if there exists a price segmentation $p_x$ for some agent feature $X$ which is optimal for the principal and yields principal value $\Pi$ and agent value $V$. Point $A$ occurs under hidden information, where the agent's additional surplus comes from their information rent. Point $B$ is attained when the principal sets the contract fully knowing the agent's costs (the principal observes $X = C$ directly). Point $C$ can be attained under a specific construction of a segmentation where the principal is held down to the hidden information value, but the outcome is still efficient so the agent receives all gains in efficiency. Such a construction can be done by iteratively and adversarially constructing each segment such that the principal is indifferent between charging the hidden information price and the segment price (See \citep{bergemann2015limits} for more details). Point $D$ also occurs from the same segmentation, where the principal chooses to give the lowest payment per segment, thus minimizing agent surplus. This is not efficent with respect to joint surplus, but still optimal for the principal because in this special segmentation, the principal is indifferent to setting any price in the support of the agents' costs in each segment.

\begin{figure}[!h]
    \centering
    \begin{tabular}{cc}
       \rotatebox{90}{Principal value, $\Pi$} & \includegraphics[width=0.5\textwidth]{figures/surplus_triangle.png} \\
       & Agent value, $V$
    \end{tabular}
    
    \caption{Surplus triangle (Figure 1 from \citep{bergemann2015limits}) showing feasible principal and agent values.}
    \label{fig:surplus-triangle}
\end{figure}

\citet{bergemann2015limits} shows that for every point in this shaded region, there exists some market segmentation (or information) that achieves this. They show that ``while additional information can never hurt the seller, it can lead social and consumer surplus to both increase, both decrease, or respectively increase and decrease.'' Still, they conclude with an open question that ``exactly which form of market segmentation arises in practice is no doubt influenced by many factors. [...] Thus, a natural and important direction for future research is to better understand which forms of price discrimination will endogenously arise, and for whose benefit.''

\subsection{Difference in our setting}

This latter question is closer to our goals, where we consider what forms of price discrimination arise when the agent has initial access to information, and gets to choose whether or not to share it. Under such a mechanism, what types of information end up benefiting society? 

In our setting, since the agent decides the revelation policy, the feasible set of $(\Pi, V)$ will instead look like the subtriangle $ACE$ in Figure \ref{fig:surplus-triangle-agent} (assuming that when the principal is indifferent between pricings, the principal defaults to choosing the pricing that also maximizes agent surplus, so the allocation is efficient). In this case, the agent will never reveal information that leads to segmentations that only yield worse value for the agent than the hidden information pricing $A$.

\snote{Question: can we characterize the types of segmentations over discrete values that yield triangle ACE?}

\begin{figure}[!h]
    \centering
    \begin{tabular}{cc}
       \rotatebox{90}{Principal value, $\Pi$} & \includegraphics[width=0.5\textwidth]{figures/surplus_triangle_agent.png} \\
       & Agent value, $V$
    \end{tabular}
    
    \caption{Surplus triangle, where subtriangle ACE shows feasible principal and agent values when the agent decides the revelation policy.}
    \label{fig:surplus-triangle-agent}
\end{figure}

\subsection{Noise trajectories}

Suppose the cost distribution $C$ is a mixture of exponentials with means $\lambda_0, \lambda_1$. The plot below shows the surplus triangle, along with a trajectory for values when the agent adds noise $\veps$.

